Power Studies For Two-sample Methods For Multivariate Data

We present the results of a large number of simulation studies regarding the power of various non-parametric two-sample tests for multivariate data. This includes both continuous and discrete data. In general no single method can be relied upon to provide good power, any one method may be quite good for some combination of null hypothesis and alternative and may fail badly for another. Based on the results of these studies we propose a fairly small number of methods chosen such that for any of the case studies included here at least one of the methods has good power. The studies were carried out using the R package MD2sample, available from CRAN.

==> tables/tblcont.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{c|c|c|c|c|c|c|c|c}\toprule
AZ &ES &EP &BF &AD &NN5 &CvM &KS &Ball\\
82.6 &80.8 &76.1 &71.5 &64.5 &63.2 &58.1 &53.8 &53\\\midrule
FR &CF1 &CF3 &K &CF4 &NN1 &CF2 &NN0 &BG\\
52.9 &52.9 &52.9 &50.2 &49.7 &43.9 &43.4 &36.1 &31.8\\\bottomrule
\end{tabular}
\caption{Mean power of tests for continuous data}
\end{table}
 
 
 
 
\begin{table}[ht]
\centering
\begin{tabular}{c|c|c|c|c|c|c|c|c}\toprule
AZ &ES &EP &BF &AD &NN5 &CvM &Ball &BG\\
74 &44 &38 &32 &30 &30 &26 &22 &16\\\midrule
K &FR &CF1 &CF3 &KS &CF2 &CF4 &NN1 &NN0\\
14 &14 &14 &14 &12 &6 &6 &2 &2\\\bottomrule
\end{tabular}
\caption{Percentage of times a test is close to best  for continuous data}
\end{table}
 
 


==> tables/tblcontall.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{c|c|c|c|c|c|c|c|c}\toprule
AZ &ES &EP &BF &AD &NN5 &CvM &KS &Ball\\
82.6 &80.8 &76.1 &71.5 &64.5 &63.2 &58.1 &53.8 &53\\\midrule
FR &CF1 &CF3 &K &CF4 &NN1 &CF2 &NN0 &BG\\
52.9 &52.9 &52.9 &50.2 &49.7 &43.9 &43.4 &36.1 &31.8\\\bottomrule
\end{tabular}
\caption{Mean power of tests for continuous data}
\end{table}
 
 
\begin{table}[ht]
\centering
\begin{tabular}{c|c|c|c|c|c|c|c|c|c}\toprule
AZ &ES &EP &BF &NN5 &FR &CF1 &CF3 &AD &CF4\\
90.3 &89.8 &85.6 &78.4 &70.1 &65.8 &65.8 &65.8 &63.2 &59.1\\\midrule
CvM &NN1 &CF2 &KS &Ball &NN0 &K &BG\\
59.1 &55.1 &51.7 &49.9 &46.9 &45.6 &41.5 &14.6\\\bottomrule
\end{tabular}
\caption{Mean power of tests for continuous two-dimensional data with equal marginals}
\end{table}
 
 
\begin{table}[ht]
\centering
\begin{tabular}{c|c|c|c|c|c|c|c|c}\toprule
AD &NN5 &CvM &AZ &KS &BF &CF4 &FR &CF1\\
81.4 &81.3 &76.6 &71.1 &55.9 &55.5 &55.2 &53.3 &53.3\\\midrule
CF3 &CF2 &NN1 &K &Ball &NN0 &BG\\
53.3 &52 &45.6 &33.4 &30.4 &19.7 &8.8\\\bottomrule
\end{tabular}
\caption{Mean power of tests for continuous five-dimensional data with equal marginals}
\end{table}
 
 
\begin{table}[ht]
\centering
\begin{tabular}{c|c|c|c|c|c|c|c|c|c}\toprule
AZ &BF &ES &K &EP &AD &Ball &NN5 &KS &FR\\
83.7 &73.3 &71.8 &69.1 &66.6 &60.8 &60.4 &58 &56 &52.5\\\midrule
CF1 &CF3 &BG &CvM &CF4 &NN1 &NN0 &CF2\\
52.5 &52.5 &49.9 &48.7 &45 &43 &39.5 &36.5\\\bottomrule
\end{tabular}
\caption{Mean power of tests for continuous two-dimensional data with unequal marginals}
\end{table}
 
 
 
 
\begin{table}[ht]
\centering
\begin{tabular}{c|c|c|c|c|c|c|c|c}\toprule
AZ &ES &EP &BF &AD &NN5 &CvM &Ball &BG\\
74 &44 &38 &32 &30 &30 &26 &22 &16\\\midrule
K &FR &CF1 &CF3 &KS &CF2 &CF4 &NN1 &NN0\\
14 &14 &14 &14 &12 &6 &6 &2 &2\\\bottomrule
\end{tabular}
\caption{Percentage of times a test is close to best  for continuous data}
\end{table}
 
 
\begin{table}[ht]
\centering
\begin{tabular}{c|c|c|c|c|c|c|c|c}\toprule
ES &AZ &EP &NN5 &FR &CF1 &CF3 &CvM &AD\\
94 &88 &82 &35 &29 &29 &29 &24 &24\\\midrule
BF &Ball &CF4 &KS &K &NN1 &NN0 &CF2 &BG\\
24 &18 &12 &6 &6 &6 &6 &6 &0\\\bottomrule
\end{tabular}
\caption{Percentage of times a test is close to best  for continuous two-dimensional data with equal marginals}
\end{table}
 
 
\begin{table}[ht]
\centering
\begin{tabular}{c|c|c|c|c|c|c|c|c}\toprule
CvM &AD &NN5 &AZ &CF2 &CF4 &K &KS &NN1\\
67 &67 &67 &44 &22 &22 &11 &0 &0\\\midrule
BF &BG &FR &NN0 &CF1 &CF3 &Ball &ES\\
0 &0 &0 &0 &0 &0 &0 &0\\\bottomrule
\end{tabular}
\caption{Percentage of times a test is close to best for continuous five-dimensional data with equal marginals}
\end{table}
 
 
\begin{table}[ht]
\centering
\begin{tabular}{c|c|c|c|c|c|c|c|c}\toprule
AZ &BF &ES &K &BG &EP &KS &AD &Ball\\
76 &41 &35 &29 &29 &29 &24 &24 &24\\\midrule
NN5 &CvM &FR &CF1 &CF3 &NN1 &NN0 &CF2 &CF4\\
18 &12 &12 &12 &12 &0 &0 &0 &0\\\bottomrule
\end{tabular}
\caption{Percentage of times a test is close to best for continuous two-dimensional data with unequal marginals}
\end{table}
 
 


==> tables/tbldisc.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{c|c|c|c|c|c|c|c}\toprule
Chisquare &NN &AD &K &KS &CvM &AZ &BF\\
79.4 &53.2 &49.2 &47.4 &43.5 &42.9 &26.5 &20.2\\\bottomrule
\end{tabular}
\caption{Mean power of tests for discrete data}
\end{table}
 
 
 
 
\begin{table}[ht]
\centering
\begin{tabular}{c|c|c|c|c|c|c|c}\toprule
Chisquare &K &KS &AD &NN &AZ &CvM &BF\\
85 &21 &15 &15 &15 &15 &9 &6\\\bottomrule
\end{tabular}
\caption{Percentage of times a test is close to best  for discrete data}
\end{table}
 
 


==> tables/tbldiscall.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{c|c|c|c|c|c|c|c}\toprule
Chisquare &NN &AD &K &KS &CvM &AZ &BF\\
79.4 &53.2 &49.2 &47.4 &43.5 &42.9 &26.5 &20.2\\\bottomrule
\end{tabular}
\caption{Mean power of tests for discrete data}
\end{table}
 
 
\begin{table}[ht]
\centering
\begin{tabular}{c|c|c|c|c|c|c|c}\toprule
Chisquare &NN &AD &CvM &KS &K &AZ &BF\\
88.8 &61.7 &48.6 &45.1 &38.4 &33.3 &12.4 &12\\\bottomrule
\end{tabular}
\caption{Mean power of tests for discrete data with equal marginals}
\end{table}
 
 
\begin{table}[ht]
\centering
\begin{tabular}{c|c|c|c|c|c|c|c}\toprule
Chisquare &K &AD &KS &NN &AZ &CvM &BF\\
70 &61.5 &49.8 &48.5 &44.6 &40.7 &40.6 &28.4\\\bottomrule
\end{tabular}
\caption{Mean power of tests for discrete data with unequal marginals}
\end{table}
 
 
 
 
\begin{table}[ht]
\centering
\begin{tabular}{c|c|c|c|c|c|c|c}\toprule
Chisquare &K &KS &AD &NN &AZ &CvM &BF\\
85 &21 &15 &15 &15 &15 &9 &6\\\bottomrule
\end{tabular}
\caption{Percentage of times a test is close to best  for discrete data}
\end{table}
 
 
\begin{table}[ht]
\centering
\begin{tabular}{c|c|c|c|c|c|c|c}\toprule
Chisquare &NN &AD &KS &K &CvM &AZ &BF\\
100 &29 &12 &6 &6 &6 &6 &6\\\bottomrule
\end{tabular}
\caption{Percentage of times a test is close to best  for discrete data with equal marginals}
\end{table}
 
 
\begin{table}[ht]
\centering
\begin{tabular}{c|c|c|c|c|c|c|c}\toprule
Chisquare &K &KS &AZ &AD &CvM &BF &NN\\
71 &35 &24 &24 &18 &12 &6 &0\\\bottomrule
\end{tabular}
\caption{Percentage of times a test is close to best for discrete data with unequal marginals}
\end{table}
 
 

